Transferability Ranking of Adversarial Examples

Adversarial transferability in black-box scenarios presents a unique challenge: while attackers can employ surrogate models to craft adversarial examples, they lack assurance on whether these examples will successfully compromise the target model. Until now, the prevalent method to ascertain success has been trial and error-testing crafted samples directly on the victim model. This approach, however, risks detection with every attempt, forcing attackers to either perfect their first try or face exposure. Our paper introduces a ranking strategy that refines the transfer attack process, enabling the attacker to estimate the likelihood of success without repeated trials on the victim's system. By leveraging a set of diverse surrogate models, our method can predict transferability of adversarial examples. This strategy can be used to either select the best sample to use in an attack or the best perturbation to apply to a specific sample. Using our strategy, we were able to raise the transferability of adversarial examples from a mere 20% - akin to random selection-up to near upper-bound levels, with some scenarios even witnessing a 100% success rate. This substantial improvement not only sheds light on the shared susceptibilities across diverse architectures but also demonstrates that attackers can forego the detectable trial-and-error tactics raising increasing the threat of surrogate-based attacks.

==> tables/archi_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ccccccc@{}}
\toprule
 & k=5 & k@20\% & k@40\% & k@60\% & k@80\% & \begin{tabular}[c]{@{}c@{}}Lower-\\bound\\(random) \end{tabular} \\ \midrule
\multicolumn{1}{|c}{w/o ET - Noise} & 1 & .994 & .988 & .977 & \multicolumn{1}{c|}{.947} & \multicolumn{1}{c|}{} \\ \cmidrule(r){1-6}
\multicolumn{1}{|c}{w/o ET - SM} & 1 & .991 & .98 & .965 & \multicolumn{1}{c|}{.945} & \multicolumn{1}{c|}{} \\ \cmidrule(r){1-6}
\multicolumn{1}{|c}{with HET} & 1 & 1 & 1 & .997 & \multicolumn{1}{c|}{.987} & \multicolumn{1}{c|}{.915} \\ \cmidrule(r){1-6}
\multicolumn{1}{|c}{\begin{tabular}[c]{@{}c@{}}with HET \\ \& Transforms\end{tabular}} & 1 & 1 & 1 & .999 & \multicolumn{1}{c|}{.992} & \multicolumn{1}{c|}{} \\ \cmidrule(r){1-6}
%\specialrule(r){1-6}{.2em}{.1em}{.1em}
\multicolumn{1}{|c}{Upper-bound} & 1 & 1 & 1 & 1 & \multicolumn{1}{c|}{1} & \multicolumn{1}{c|}{} \\ \bottomrule
\end{tabular}%
}
\caption{\textbf{E1.4} - Transfer success rates when the attacker and victim use different model architectures. Here $k@$\textit{percentile} stands for the $k$ at the value that equals to the percentile of the size of the dataset.}
\label{Archi_table}
\end{table}

==> tables/atk_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[t]
\caption{\textbf{E1.4} Transfer success rates when using different attack algorithms. Here $k@$\textit{percentile} stands for the $k$ at the value that equals to the percentile with respect to the size of the dataset.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccccc@{}}
\toprule
 & k=5 & k@20\% & k@40\% & k@60\% & k@80\% & \begin{tabular}[c]{@{}c@{}}Lower-\\ bound\\ (random)\end{tabular} \\ \midrule
 & \multicolumn{5}{c|}{without ET - Noise / without ET - SM / with HET // Upper-bound} &  \\ \midrule
\multicolumn{1}{|c}{FGSM} & .991 / .981 / 1 // 1 & .884 / .884 / .996 // 1 & .798 / .81 / .959 // .984 & .711 / .726 / .854 // .873 & \multicolumn{1}{c|}{.623 / .642 / .69 // .694} & \multicolumn{1}{c|}{.555} \\ \midrule
\multicolumn{1}{|c}{PGD} & 1 / 1 / 1 // 1 & .997 / .994 / 1 // 1 & .992 / .986 / 1 // 1 & .982 / .97 / .999 // 1 & \multicolumn{1}{c|}{.95 / 95 / .993 // .999} & \multicolumn{1}{c|}{.92} \\ \midrule
\multicolumn{1}{|c}{\begin{tabular}[c]{@{}c@{}}PGD+\\ Momentum\end{tabular}} & 1 / 1 / 1 // 1 & .999 / .997 / 1 // 1 & .995 / .991 / 1 // 1 & .99 / .979 / 1 // 1 & \multicolumn{1}{c|}{.964 / .964 / .997 // 1} & \multicolumn{1}{c|}{.939} \\ \midrule
\multicolumn{1}{|c}{\begin{tabular}[c]{@{}c@{}}PGD+\\ Input\\ diversity\end{tabular}} & 1 / 1 / 1 // 1 & .997 / .995 / 1 // 1 & .993 / .989 / 1 // 1 & .986 / .976 / 1 // 1 & \multicolumn{1}{c|}{.959 / .958 / .996 // 1} & \multicolumn{1}{c|}{.931} \\ \bottomrule
\end{tabular}%
}

\label{atk_table}
\end{table*}

==> tables/pertubation_ranking/pertubation_ranking_imagenet_cifar.tex <==

\begin{table}[]


\resizebox{\linewidth}{!}{%

\begin{tabular}{|ccc|l|lll|lll|lll|lll|}
\hline
\multicolumn{3}{|c|}{}                                                                                                             & \multicolumn{1}{c|}{}                           & \multicolumn{3}{c|}{SoftMax}                                                             & \multicolumn{3}{c|}{SoftMax+Noise}                                                      & \multicolumn{3}{c|}{HET}                                                                 & \multicolumn{3}{c|}{Upper B.}                                                                 \\ \cline{5-16} 
                                                  & Surrogate                                               & Victim               & \multicolumn{1}{c|}{\multirow{-2}{*}{Lower B.}} & \multicolumn{1}{c}{5\%}     & \multicolumn{1}{c}{10\%}    & \multicolumn{1}{c|}{20\%}    & \multicolumn{1}{c}{5\%}     & \multicolumn{1}{c}{10\%}    & \multicolumn{1}{c|}{20\%}    & \multicolumn{1}{c}{5\%}     & \multicolumn{1}{c}{10\%}    & \multicolumn{1}{c|}{20\%}    & \multicolumn{1}{c}{5\%}      & \multicolumn{1}{c}{10\%}      & \multicolumn{1}{c|}{20\%}      \\ \hline
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ViT\_l\_16           & \cellcolor[HTML]{FCC17C}0.34                    & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FBAA77}0.25 & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FCC47C}0.35 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{83C77D}0.9  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet121          & \cellcolor[HTML]{FCB479}0.29                    & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2  & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FCC47C}0.35 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{92CC7E}0.85 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Efficientnet-b2     & \cellcolor[HTML]{FBAC78}0.26                    & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FCB77A}0.3 & \cellcolor[HTML]{FBAA77}0.25 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FCB77A}0.3 & \cellcolor[HTML]{FCC47C}0.35 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{A2D07F}0.8  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Resnet18             & \cellcolor[HTML]{FDC97D}0.37                    & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FBAA77}0.25 & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{C1DA81}0.7 & \cellcolor[HTML]{FFEB84}0.5  & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{92CC7E}0.85 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{\multirow{-5}{*}{ViT\_b\_16}}       & Swin\_s              & \cellcolor[HTML]{FA9D75}0.2                     & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FA9072}0.15 & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8766D}0.05 & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{F0E784}0.55 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ViT\_b\_16           & \cellcolor[HTML]{FBA476}0.23                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{F98370}0.1  & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F98370}0.1 & \cellcolor[HTML]{FA9072}0.15 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{83C77D}0.9 & \cellcolor[HTML]{D1DE82}0.65 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet161          & \cellcolor[HTML]{FCC17C}0.34                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{F98370}0.1  & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F98370}0.1 & \cellcolor[HTML]{FA9072}0.15 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{83C77D}0.9  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Efficientnet-b2     & \cellcolor[HTML]{FBAF78}0.27                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FCB77A}0.3 & \cellcolor[HTML]{FA9072}0.15 & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2  & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{B1D580}0.75 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Resnet18             & \cellcolor[HTML]{FEDE81}0.45                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FCB77A}0.3 & \cellcolor[HTML]{FBAA77}0.25 & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FDD17F}0.4  & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{83C77D}0.9 & \cellcolor[HTML]{83C77D}0.9  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{\multirow{-5}{*}{DenseNet121}}      & Swin\_s              & \cellcolor[HTML]{FA9774}0.18                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F98370}0.1 & \cellcolor[HTML]{F8766D}0.05 & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F98370}0.1  & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{D1DE82}0.65 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{7EC67D}0.915  \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ViT\_b\_16           & \cellcolor[HTML]{FBA276}0.22                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{F98370}0.1 & \cellcolor[HTML]{F98370}0.1  & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{92CC7E}0.85 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet121          & \cellcolor[HTML]{FCC17C}0.34                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FBAA77}0.25 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FCC47C}0.35 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{73C37C}0.95 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Efficientnet\_b1     & \cellcolor[HTML]{FDC67D}0.36                    & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FCB77A}0.3 & \cellcolor[HTML]{FA9D75}0.2  & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FBAA77}0.25 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{92CC7E}0.85 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Resnet18             & \cellcolor[HTML]{FED880}0.43                    & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{FFEB84}0.5 & \cellcolor[HTML]{FDD17F}0.4  & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{FFEB84}0.5 & \cellcolor[HTML]{FFEB84}0.5  & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{83C77D}0.9 & \cellcolor[HTML]{83C77D}0.9  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{\multirow{-5}{*}{Efficientnet-b2}} & Swin\_s              & \cellcolor[HTML]{FA9D75}0.2                     & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8766D}0.05 & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{C1DA81}0.7 & \cellcolor[HTML]{C1DA81}0.7  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{6FC27C}0.9625 \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ViT\_b\_16           & \cellcolor[HTML]{FBA476}0.23                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F98370}0.1  & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{F98370}0.1 & \cellcolor[HTML]{F98370}0.1  & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{83C77D}0.9 & \cellcolor[HTML]{B1D580}0.75 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet121          & \cellcolor[HTML]{FCBE7B}0.33                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2  & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FCB77A}0.3 & \cellcolor[HTML]{FBAA77}0.25 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{83C77D}0.9 & \cellcolor[HTML]{83C77D}0.9  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Efficientnet-b2     & \cellcolor[HTML]{FBAA77}0.25                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F98370}0.1 & \cellcolor[HTML]{F98370}0.1  & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{F98370}0.1  & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{C1DA81}0.7  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Resnet34             & \cellcolor[HTML]{FCC47C}0.35                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FBAA77}0.25 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9072}0.15 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{83C77D}0.9 & \cellcolor[HTML]{92CC7E}0.85 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{\multirow{-5}{*}{Resnet18}}         & Swin\_s              & \cellcolor[HTML]{FA9573}0.17                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8766D}0.05 & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8766D}0.05 & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{C1DA81}0.7 & \cellcolor[HTML]{E0E383}0.6  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{8FCB7E}0.86   \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ViT\_b\_16           & \cellcolor[HTML]{FBA777}0.24                    & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FFEB84}0.5 & \cellcolor[HTML]{FCC47C}0.35 & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2  & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{C1DA81}0.7  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet121          & \cellcolor[HTML]{FCB479}0.29                    & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{FFEB84}0.5 & \cellcolor[HTML]{FCC47C}0.35 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FCB77A}0.3 & \cellcolor[HTML]{FCC47C}0.35 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{83C77D}0.9  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Efficientnet-b2     & \cellcolor[HTML]{FBAA77}0.25                    & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{FDD17F}0.4  & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FCB77A}0.3 & \cellcolor[HTML]{FA9D75}0.2  & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{83C77D}0.9 & \cellcolor[HTML]{B1D580}0.75 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Resnet18             & \cellcolor[HTML]{FDC97D}0.37                    & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{FFEB84}0.5 & \cellcolor[HTML]{FEDE81}0.45 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FCB77A}0.3 & \cellcolor[HTML]{FCC47C}0.35 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{92CC7E}0.85 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{\multirow{-25}{*}{Imagenet}} & \multicolumn{1}{c|}{\multirow{-5}{*}{Swin\_s}}          & Swin\_t              & \cellcolor[HTML]{F3E884}0.54                    & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{C1DA81}0.7 & \cellcolor[HTML]{FFEB84}0.5  & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FDD17F}0.4  & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\ \hline
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ViT             & \cellcolor[HTML]{F8736D}0.04                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8766D}0.05 & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9072}0.15 & \cellcolor[HTML]{8CCA7E}0.87 & \cellcolor[HTML]{FEE482}0.475 & \cellcolor[HTML]{FBA676}0.2375 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet121          & \cellcolor[HTML]{B8D780}0.73                    & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{C1DA81}0.7  & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{C1DA81}0.7 & \cellcolor[HTML]{B1D580}0.75 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{73C37C}0.95 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Efficientnet-b0       & \cellcolor[HTML]{F9806F}0.09                    & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{F98370}0.1 & \cellcolor[HTML]{F98370}0.1  & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{F98370}0.1 & \cellcolor[HTML]{FA9072}0.15 & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FBAA77}0.25 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{99CE7F}0.83  & \cellcolor[HTML]{FDD47F}0.415  \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Resnet18             & \cellcolor[HTML]{F86E6C}0.02                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{F98370}0.1 & \cellcolor[HTML]{F8766D}0.05 & \cellcolor[HTML]{FDD680}0.42 & \cellcolor[HTML]{FA9F75}0.21  & \cellcolor[HTML]{F98470}0.105  \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{\multirow{-5}{*}{ViT}}              & Swin\_s              & \cellcolor[HTML]{FA9774}0.18                    & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2  & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F98370}0.1 & \cellcolor[HTML]{FBAA77}0.25 & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{F0E784}0.55 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{7FC67D}0.9125 \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ViT                  & \cellcolor[HTML]{FBA476}0.23                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F98370}0.1 & \cellcolor[HTML]{FBAA77}0.25 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2  & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{FFEB84}0.5 & \cellcolor[HTML]{FFEB84}0.5  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{64BF7C}0.9975 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet121     & \cellcolor[HTML]{CADC81}0.67                    & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{C1DA81}0.7 & \cellcolor[HTML]{B1D580}0.75 & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{FFEB84}0.5 & \cellcolor[HTML]{FFEB84}0.5  & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{83C77D}0.9 & \cellcolor[HTML]{B1D580}0.75 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Efficientnet-b0       & \cellcolor[HTML]{FBB179}0.28                    & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{F98370}0.1 & \cellcolor[HTML]{FCC47C}0.35 & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FCC47C}0.35 & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{C1DA81}0.7 & \cellcolor[HTML]{C1DA81}0.7  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{67BF7C}0.99   \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Resnet18             & \cellcolor[HTML]{FCC47C}0.35                    & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FCB77A}0.3 & \cellcolor[HTML]{FEDE81}0.45 & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{FFEB84}0.5 & \cellcolor[HTML]{FFEB84}0.5  & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{FFEB84}0.5  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{64BF7C}0.9975 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{\multirow{-5}{*}{DenseNet121}}      & Swin\_s              & \cellcolor[HTML]{F98D72}0.14                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F98370}0.1 & \cellcolor[HTML]{FA9072}0.15 & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{F98370}0.1  & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FFEB84}0.5 & \cellcolor[HTML]{FCC47C}0.35 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{C5DB81}0.6875 \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ViT                  & \cellcolor[HTML]{FBAA77}0.25                    & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FCC47C}0.35 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FBAA77}0.25 & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{FFEB84}0.5  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet121          & \cellcolor[HTML]{D1DE82}0.65                    & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{83C77D}0.9 & \cellcolor[HTML]{B1D580}0.75 & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{D1DE82}0.65 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{83C77D}0.9 & \cellcolor[HTML]{73C37C}0.95 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Efficientnet-b0  & \cellcolor[HTML]{FCBC7B}0.32                    & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FFEB84}0.5 & \cellcolor[HTML]{F0E784}0.55 & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FFEB84}0.5 & \cellcolor[HTML]{FDD17F}0.4  & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{D1DE82}0.65 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Resnet18             & \cellcolor[HTML]{FDCB7E}0.38                    & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{C1DA81}0.7 & \cellcolor[HTML]{D1DE82}0.65 & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{C1DA81}0.7 & \cellcolor[HTML]{FFEB84}0.5  & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{83C77D}0.9 & \cellcolor[HTML]{A2D07F}0.8  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{\multirow{-5}{*}{Efficientnet-b0}}   & Swin\_s              & \cellcolor[HTML]{FA9072}0.15                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FA9D75}0.2  & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2  & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{FEDE81}0.45 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{ABD380}0.77   \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ViT                  & \cellcolor[HTML]{FBA276}0.22                    & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{F98370}0.1 & \cellcolor[HTML]{FA9072}0.15 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FCB77A}0.3  & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{FFEB84}0.5  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{64BF7C}0.9975 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet121          & \cellcolor[HTML]{FBB179}0.28                    & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FCB77A}0.3 & \cellcolor[HTML]{FA9D75}0.2  & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FCB77A}0.3  & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{83C77D}0.9 & \cellcolor[HTML]{C1DA81}0.7  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{6BC17C}0.975  \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Efficientnet-b0       & \cellcolor[HTML]{FBA777}0.24                    & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2  & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FCC47C}0.35 & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{D1DE82}0.65 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{6BC17C}0.975 & \cellcolor[HTML]{80C77D}0.91   \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Resnet18        & \cellcolor[HTML]{FA9D75}0.2                     & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FCB77A}0.3  & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FCB77A}0.3 & \cellcolor[HTML]{FCB77A}0.3  & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{FFEB84}0.5 & \cellcolor[HTML]{F0E784}0.55 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{6AC07C}0.98  & \cellcolor[HTML]{93CC7E}0.8475 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{\multirow{-5}{*}{Resnet18}}         & Swin\_s              & \cellcolor[HTML]{F98570}0.11                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F98370}0.1 & \cellcolor[HTML]{FA9072}0.15 & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{FEDE81}0.45 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{72C37C}0.955 & \cellcolor[HTML]{F5E884}0.535  \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ViT                  & \cellcolor[HTML]{FCC17C}0.34                    & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{FFEB84}0.5 & \cellcolor[HTML]{FDD17F}0.4  & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FCB77A}0.3  & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{C1DA81}0.7 & \cellcolor[HTML]{F0E784}0.55 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet121          & \cellcolor[HTML]{F6E984}0.53                    & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{FFEB84}0.5 & \cellcolor[HTML]{FFEB84}0.5  & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FFEB84}0.5  & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{83C77D}0.9  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Efficientnet-b0       & \cellcolor[HTML]{F98A71}0.13                    & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{F98370}0.1 & \cellcolor[HTML]{F98370}0.1  & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{F98370}0.1 & \cellcolor[HTML]{FA9072}0.15 & \cellcolor[HTML]{A2D07F}0.8 & \cellcolor[HTML]{E0E383}0.6 & \cellcolor[HTML]{FDD17F}0.4  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{CADC81}0.6725 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & Resnet18             & \cellcolor[HTML]{FA9573}0.17                    & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FCB77A}0.3  & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9072}0.15 & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FCC47C}0.35 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1     & \cellcolor[HTML]{A1D07F}0.8025 \\
\multicolumn{1}{|c|}{\multirow{-25}{*}{Cifar}}    & \multicolumn{1}{c|}{\multirow{-5}{*}{Swin\_s}}           & Swin\_s         & \cellcolor[HTML]{F9806F}0.09                    & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{F98370}0.1  & \cellcolor[HTML]{FA9D75}0.2 & \cellcolor[HTML]{F98370}0.1 & \cellcolor[HTML]{F98370}0.1  & \cellcolor[HTML]{FDD17F}0.4 & \cellcolor[HTML]{FFEB84}0.5 & \cellcolor[HTML]{FBAA77}0.25 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{87C97E}0.885 & \cellcolor[HTML]{FEDC81}0.445  \\ \hline
\end{tabular}
}
\caption{The average transferability of a sample when ranking its potential perturbations for the CIFAR10 and ImageNet datasets over 100 trials. Columns represent the various ranking methods, and rows indicate the combination of victim and surrogate model architectures, ensuring that \( F_0 \) is chosen from architectures different from the victim's.}\label{tab:E2.1A}
\end{table}

==> tables/pertubation_ranking/pertubation_ranking_xray_road_sign.tex <==
\begin{table}[]
\resizebox{\linewidth}{!}{%

\begin{tabular}{|ccc|l|lll|lll|lll|lll|}
\hline
\multicolumn{3}{|c|}{}                                                                                                          & \multicolumn{1}{c|}{}                           & \multicolumn{3}{c|}{SoftMax}                                                             & \multicolumn{3}{c|}{SoftMax+Noise}                                                             & \multicolumn{3}{c|}{HET}                                                                 & \multicolumn{3}{c|}{Upper B.}                                                                \\ \cline{5-16} 
                                                   & Sorrogate                                               & Victim           & \multicolumn{1}{c|}{\multirow{-2}{*}{Lower B.}} & \multicolumn{1}{c}{5\%}     & \multicolumn{1}{c}{10\%}    & \multicolumn{1}{c|}{20\%}    & \multicolumn{1}{c}{5\%}     & \multicolumn{1}{c}{10\%}    & \multicolumn{1}{c|}{20\%}    & \multicolumn{1}{c}{5\%}     & \multicolumn{1}{c}{10\%}    & \multicolumn{1}{c|}{20\%}    & \multicolumn{1}{c}{5\%}      & \multicolumn{1}{c}{10\%}     & \multicolumn{1}{c|}{20\%}      \\ \hline
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{DCE182}0.42                    & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{CCDD82}0.5 & \cellcolor[HTML]{CCDD82}0.5  & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{D6E082}0.45 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{78C47D}0.9 & \cellcolor[HTML]{6EC27C}0.95 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{F5E984}0.3                     & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{FCB77A}0.15 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{98CE7F}0.75 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet-b2 & \cellcolor[HTML]{F3E884}0.31                    & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{FCB77A}0.15 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{83C87D}0.85 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{FFEB84}0.25                    & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{F5E984}0.3 & \cellcolor[HTML]{FCB77A}0.15 & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{F5E984}0.3 & \cellcolor[HTML]{FFEB84}0.25 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{8DCA7E}0.8 & \cellcolor[HTML]{ACD480}0.65 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{\multirow{-5}{*}{ViT}}              & Swin\_s          & \cellcolor[HTML]{FEE583}0.24                    & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{F5E984}0.3 & \cellcolor[HTML]{F5E984}0.3  & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{F5E984}0.3 & \cellcolor[HTML]{FFEB84}0.25 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{78C47D}0.9 & \cellcolor[HTML]{ACD480}0.65 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{FDD680}0.21                    & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FFEB84}0.25 & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F5E984}0.3 & \cellcolor[HTML]{FFEB84}0.25 & \cellcolor[HTML]{8DCA7E}0.8 & \cellcolor[HTML]{A2D07F}0.7 & \cellcolor[HTML]{CCDD82}0.5  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{93CC7E}0.77                    & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{8DCA7E}0.8 & \cellcolor[HTML]{8DCA7E}0.8  & \cellcolor[HTML]{8DCA7E}0.8 & \cellcolor[HTML]{78C47D}0.9 & \cellcolor[HTML]{78C47D}0.9  & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet-b2 & \cellcolor[HTML]{E2E383}0.39                    & \cellcolor[HTML]{8DCA7E}0.8 & \cellcolor[HTML]{CCDD82}0.5 & \cellcolor[HTML]{E0E383}0.4  & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{CCDD82}0.5 & \cellcolor[HTML]{E0E383}0.4  & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{78C47D}0.9 & \cellcolor[HTML]{8DCA7E}0.8  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{E2E383}0.39                    & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{CCDD82}0.5  & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{CCDD82}0.5 & \cellcolor[HTML]{E0E383}0.4  & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{8DCA7E}0.8 & \cellcolor[HTML]{8DCA7E}0.8  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{\multirow{-5}{*}{DenseNet121}}      & Swin\_s          & \cellcolor[HTML]{FDD680}0.21                    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{8DCA7E}0.8 & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{D6E082}0.45 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{66BF7C}0.99   \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{FDD680}0.21                    & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{F5E984}0.3  & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{8DCA7E}0.8 & \cellcolor[HTML]{8DCA7E}0.8 & \cellcolor[HTML]{CCDD82}0.5  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{65BF7C}0.9925 \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet-b2 & \cellcolor[HTML]{FDEB84}0.26                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{FFEB84}0.25 & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{F5E984}0.3 & \cellcolor[HTML]{FFEB84}0.25 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{78C47D}0.9 & \cellcolor[HTML]{A2D07F}0.7  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{63BE7B}1                       & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{FFEB84}0.25                    & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{F5E984}0.3 & \cellcolor[HTML]{EBE683}0.35 & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{CCDD82}0.5 & \cellcolor[HTML]{E0E383}0.4  & \cellcolor[HTML]{8DCA7E}0.8 & \cellcolor[HTML]{8DCA7E}0.8 & \cellcolor[HTML]{CCDD82}0.5  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{\multirow{-5}{*}{Efficientnet-b2}} & Swin\_s          & \cellcolor[HTML]{FDCB7E}0.19                    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{FCB77A}0.15 & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{EBE683}0.35 & \cellcolor[HTML]{8DCA7E}0.8 & \cellcolor[HTML]{A2D07F}0.7 & \cellcolor[HTML]{C1D981}0.55 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{7AC57D}0.89   \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{FDD680}0.21                    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FCB77A}0.15 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{8DCA7E}0.8 & \cellcolor[HTML]{C1D981}0.55 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{D2DE82}0.47                    & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{EBE683}0.35 & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{F5E984}0.3 & \cellcolor[HTML]{EBE683}0.35 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{78C47D}0.9 & \cellcolor[HTML]{8DCA7E}0.8  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{D6E082}0.45                    & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{CCDD82}0.5 & \cellcolor[HTML]{B7D780}0.6  & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{D6E082}0.45 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{78C47D}0.9 & \cellcolor[HTML]{8DCA7E}0.8  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet-b2 & \cellcolor[HTML]{68C07C}0.98                    & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{\multirow{-5}{*}{Resnet18}}         & Swin\_s          & \cellcolor[HTML]{FEE583}0.24                    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FFEB84}0.25 & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{B7D780}0.6  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{65BF7C}0.995  \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{FEE583}0.24                    & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{F5E984}0.3 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{D6E082}0.45 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{8DCA7E}0.8 & \cellcolor[HTML]{B7D780}0.6  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{E4E483}0.38                    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{F5E984}0.3 & \cellcolor[HTML]{F5E984}0.3  & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{D6E082}0.45 & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{8DCA7E}0.8 & \cellcolor[HTML]{A2D07F}0.7  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{D6E082}0.45                    & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{E0E383}0.4  & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{F5E984}0.3 & \cellcolor[HTML]{CCDD82}0.5  & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{6EC27C}0.95 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet-b2 & \cellcolor[HTML]{EFE784}0.33                    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FFEB84}0.25 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FFEB84}0.25 & \cellcolor[HTML]{8DCA7E}0.8 & \cellcolor[HTML]{A2D07F}0.7 & \cellcolor[HTML]{C1D981}0.55 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{\multirow{-25}{*}{X-Ray}}     & \multicolumn{1}{c|}{\multirow{-5}{*}{Swin\_s}}          & Swin\_s          & \cellcolor[HTML]{66BF7C}0.99                    & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\ \hline
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{F86E6C}0.01                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{F98370}0.05 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{F98370}0.05   \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{F86E6C}0.01                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{F98370}0.05 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{F98370}0.05   \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet-b2 & \cellcolor[HTML]{F97D6F}0.04                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{F5E984}0.3 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{8DCA7E}0.8  & \cellcolor[HTML]{E0E383}0.4  & \cellcolor[HTML]{FDD17F}0.2    \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{F86E6C}0.01                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{F98370}0.05 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{F98370}0.05   \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{\multirow{-5}{*}{ViT}}              & Swin\_s          & \cellcolor[HTML]{F8736D}0.02                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{E0E383}0.4  & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FA9D75}0.1    \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{F86E6C}0.01                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{F98370}0.05 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{F98370}0.05   \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{FDC67D}0.18                    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F98370}0.05 & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{CCDD82}0.5 & \cellcolor[HTML]{EBE683}0.35 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{85C87D}0.8375 \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet-b2 & \cellcolor[HTML]{F98871}0.06                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{CCDD82}0.5 & \cellcolor[HTML]{F5E984}0.3  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{B7D780}0.6  & \cellcolor[HTML]{F5E984}0.3    \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{F8736D}0.02                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{E0E383}0.4  & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FA9D75}0.1    \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{\multirow{-5}{*}{DenseNet121}}      & Swin\_s          & \cellcolor[HTML]{F8736D}0.02                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{E0E383}0.4  & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FA9D75}0.1    \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{F86E6C}0.01                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F98370}0.05 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{F98370}0.05 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{F98370}0.05   \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{F86E6C}0.01                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F98370}0.05 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{F98370}0.05 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{F98370}0.05   \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet-b2 & \cellcolor[HTML]{C5DB81}0.53                    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{F5E984}0.3 & \cellcolor[HTML]{F5E984}0.3  & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{A2D07F}0.7  & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{78C47D}0.9 & \cellcolor[HTML]{98CE7F}0.75 & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{F8736D}0.02                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{F1E784}0.32 & \cellcolor[HTML]{FCBC7B}0.16 & \cellcolor[HTML]{FA9273}0.08   \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{\multirow{-5}{*}{Efficientnet-b2}} & Swin\_s          & \cellcolor[HTML]{F8736D}0.02                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{E0E383}0.4  & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FA9D75}0.1    \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{F86E6C}0.01                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{F98370}0.05 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{F98370}0.05   \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{F86E6C}0.01                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{F98370}0.05 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{F98370}0.05   \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet-b2 & \cellcolor[HTML]{F98871}0.06                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{CCDD82}0.5 & \cellcolor[HTML]{F5E984}0.3  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{B3D580}0.62 & \cellcolor[HTML]{F3E884}0.31   \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{F1E784}0.32                    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{63BE7B}1   & \cellcolor[HTML]{78C47D}0.9 & \cellcolor[HTML]{A2D07F}0.7  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{\multirow{-5}{*}{Resnet18}}         & Swin\_s          & \cellcolor[HTML]{F8736D}0.02                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{E0E383}0.4  & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FA9D75}0.1    \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{F86E6C}0.01                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{F98370}0.05 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{F98370}0.05   \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{F86E6C}0.01                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1 & \cellcolor[HTML]{F98370}0.05 & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{F98370}0.05   \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet-b2 & \cellcolor[HTML]{F98871}0.06                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{8DCA7E}0.8 & \cellcolor[HTML]{CCDD82}0.5 & \cellcolor[HTML]{F5E984}0.3  & \cellcolor[HTML]{6AC07C}0.97 & \cellcolor[HTML]{B9D780}0.59 & \cellcolor[HTML]{F6E984}0.295  \\
\multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{F8736D}0.02                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{E0E383}0.4 & \cellcolor[HTML]{FDD17F}0.2 & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{E0E383}0.4  & \cellcolor[HTML]{FDD17F}0.2  & \cellcolor[HTML]{FA9D75}0.1    \\
\multicolumn{1}{|c|}{\multirow{-25}{*}{Road Sign}} & \multicolumn{1}{c|}{\multirow{-5}{*}{Swin\_s}}          & Swin\_s          & \cellcolor[HTML]{FDD680}0.21                    & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{FA9D75}0.1  & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0   & \cellcolor[HTML]{F8696B}0    & \cellcolor[HTML]{8DCA7E}0.8 & \cellcolor[HTML]{B7D780}0.6 & \cellcolor[HTML]{CCDD82}0.5  & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1    & \cellcolor[HTML]{63BE7B}1      \\ \hline
\end{tabular}
}
\caption{The average transferability of a sample when ranking its potential perturbations for the X-Ray and Road Sign datasets over 100 trials. Columns represent the various ranking methods, and rows indicate the combination of victim and surrogate model architectures, ensuring that \( F_0 \) is chosen from architectures different from the victim's.}\label{tab:E2.1B}
\end{table}

==> tables/scenario2_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{\textbf{E2.1} and \textbf{E2.2} - Transfer success rates when selecting the top 1 \textit{pertubation} per sample. Results are averaged over the test dataset. Values in parenthesis are the standard deviation. The transforms strategy is irrelevant when no transformation are done (\textit{Natural} and \textit{Different architecture}).}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{@{}ccccc@{}}
\toprule
Strategy & \textit{Natural} & \textit{Compressed} & \textit{Resized} & \begin{tabular}[c]{@{}c@{}}\textit{Different} \\ \textit{architecture}\end{tabular} \\ \midrule
\multicolumn{1}{|c}{Random} & .811 (.2) & .354 (.15) & .355 (.02) & \multicolumn{1}{c|}{.815 (.01)} \\ \midrule
\multicolumn{1}{|c}{w/o ET - SM} & .839 & .324 & .347 & \multicolumn{1}{c|}{.84} \\ \midrule
\multicolumn{1}{|c}{with HET} & .89 & .357 & .37 & \multicolumn{1}{c|}{.882} \\ \midrule
\multicolumn{1}{|c}{\begin{tabular}[c]{@{}c@{}} with HET\\ \& Transforms\end{tabular}} & - & .524 & .442 & \multicolumn{1}{c|}{-} \\ %\specialrule{.2em}{.1em}{.1em} 
\midrule
\multicolumn{1}{|c}{Upper-bound} & .946 & .634 & .522 & \multicolumn{1}{c|}{.946} \\ \bottomrule
\end{tabular}%
}
\label{scenario2}
\end{table}

==> tables/transforms_cifar_imagenet.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\resizebox{\linewidth}{!}{%

\begin{tabular}{|lcc|lll|lll|lll|}
\hline
\multicolumn{2}{|l}{}                                                                                       &                  & \multicolumn{3}{c|}{@5\%}                                                                        & \multicolumn{3}{c|}{@10\%}                                                                       & \multicolumn{3}{c|}{@20\%}                                                                       \\ \cline{4-12} 
                                                  & Surrogate                                               & Victim           & \multicolumn{1}{c}{Resize}     & \multicolumn{1}{c}{Comp}       & \multicolumn{1}{c|}{Comb}      & \multicolumn{1}{c}{Resize}     & \multicolumn{1}{c}{Comp}       & \multicolumn{1}{c|}{Comb}      & \multicolumn{1}{c}{Resize}     & \multicolumn{1}{c}{Comp}       & \multicolumn{1}{c|}{Comb}      \\ \hline
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & ViT\_l\_16       & \cellcolor[HTML]{6DC17C}0.9929 & \cellcolor[HTML]{6DC17C}0.9929 & \cellcolor[HTML]{6EC27C}0.9919 & \cellcolor[HTML]{82C77D}0.9782 & \cellcolor[HTML]{7FC67D}0.9807 & \cellcolor[HTML]{81C77D}0.9789 & \cellcolor[HTML]{BED981}0.9378 & \cellcolor[HTML]{BFD981}0.9368 & \cellcolor[HTML]{C3DA81}0.9344 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{68C07C}0.9959 & \cellcolor[HTML]{6AC07C}0.9944 & \cellcolor[HTML]{66BF7C}0.9975 & \cellcolor[HTML]{78C47D}0.9853 & \cellcolor[HTML]{7BC57D}0.9833 & \cellcolor[HTML]{73C37C}0.9888 & \cellcolor[HTML]{A7D27F}0.9531 & \cellcolor[HTML]{B5D680}0.9439 & \cellcolor[HTML]{9BCE7F}0.9618 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & Efficientnet\_b2 & \cellcolor[HTML]{67C07C}0.9964 & \cellcolor[HTML]{70C27C}0.9909 & \cellcolor[HTML]{6DC17C}0.9929 & \cellcolor[HTML]{8ACA7E}0.9731 & \cellcolor[HTML]{8ECB7E}0.9703 & \cellcolor[HTML]{86C87D}0.9756 & \cellcolor[HTML]{E5E483}0.9112 & \cellcolor[HTML]{EDE683}0.9058 & \cellcolor[HTML]{D9E082}0.9193 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{65BF7C}0.9980 & \cellcolor[HTML]{65BF7C}0.9980 & \cellcolor[HTML]{65BF7C}0.9980 & \cellcolor[HTML]{72C37C}0.9891 & \cellcolor[HTML]{70C27C}0.9904 & \cellcolor[HTML]{6DC17C}0.9924 & \cellcolor[HTML]{A3D17F}0.9559 & \cellcolor[HTML]{AAD380}0.9515 & \cellcolor[HTML]{97CD7E}0.9644 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{\multirow{-5}{*}{ViT\_b\_16}}       & Swin\_s          & \cellcolor[HTML]{B2D580}0.9462 & \cellcolor[HTML]{98CE7F}0.9635 & \cellcolor[HTML]{9ACE7F}0.9619 & \cellcolor[HTML]{ECE683}0.9064 & \cellcolor[HTML]{D8E082}0.9201 & \cellcolor[HTML]{C7DB81}0.9315 & \cellcolor[HTML]{FED980}0.8278 & \cellcolor[HTML]{FEDD81}0.8450 & \cellcolor[HTML]{FEE282}0.8621 \\ \cline{2-12} 
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & ViT\_b\_16       & \cellcolor[HTML]{92CC7E}0.9674 & \cellcolor[HTML]{93CC7E}0.9666 & \cellcolor[HTML]{81C77D}0.9791 & \cellcolor[HTML]{D5DF82}0.9222 & \cellcolor[HTML]{E0E283}0.9150 & \cellcolor[HTML]{BCD881}0.9389 & \cellcolor[HTML]{FDD17F}0.7986 & \cellcolor[HTML]{FDCF7E}0.7923 & \cellcolor[HTML]{FDD880}0.8254 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet161      & \cellcolor[HTML]{67BF7C}0.9968 & \cellcolor[HTML]{6CC17C}0.9932 & \cellcolor[HTML]{68C07C}0.9960 & \cellcolor[HTML]{7AC57D}0.9835 & \cellcolor[HTML]{7DC67D}0.9821 & \cellcolor[HTML]{76C47D}0.9867 & \cellcolor[HTML]{C2DA81}0.9351 & \cellcolor[HTML]{D5DF82}0.9220 & \cellcolor[HTML]{C5DB81}0.9329 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & Efficientnet\_b2 & \cellcolor[HTML]{76C47D}0.9867 & \cellcolor[HTML]{75C47D}0.9871 & \cellcolor[HTML]{72C37C}0.9891 & \cellcolor[HTML]{99CE7F}0.9626 & \cellcolor[HTML]{9DCF7F}0.9604 & \cellcolor[HTML]{91CC7E}0.9680 & \cellcolor[HTML]{FEE883}0.8837 & \cellcolor[HTML]{FEE582}0.8744 & \cellcolor[HTML]{FEE983}0.8875 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{6DC17C}0.9924 & \cellcolor[HTML]{6BC17C}0.9940 & \cellcolor[HTML]{6AC17C}0.9944 & \cellcolor[HTML]{84C87D}0.9773 & \cellcolor[HTML]{82C77D}0.9785 & \cellcolor[HTML]{80C77D}0.9795 & \cellcolor[HTML]{C9DC81}0.9303 & \cellcolor[HTML]{D4DF82}0.9228 & \cellcolor[HTML]{C6DB81}0.9325 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{\multirow{-5}{*}{DenseNet121}}      & Swin\_s          & \cellcolor[HTML]{97CD7E}0.9642 & \cellcolor[HTML]{90CB7E}0.9686 & \cellcolor[HTML]{82C77D}0.9787 & \cellcolor[HTML]{F0E784}0.9039 & \cellcolor[HTML]{CCDD82}0.9287 & \cellcolor[HTML]{BCD881}0.9389 & \cellcolor[HTML]{FDCF7E}0.7940 & \cellcolor[HTML]{FDD57F}0.8144 & \cellcolor[HTML]{FEDE81}0.8460 \\ \cline{2-12} 
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & ViT\_b\_16       & \cellcolor[HTML]{8FCB7E}0.9695 & \cellcolor[HTML]{94CC7E}0.9665 & \cellcolor[HTML]{81C77D}0.9794 & \cellcolor[HTML]{CDDD82}0.9275 & \cellcolor[HTML]{DFE283}0.9155 & \cellcolor[HTML]{BAD780}0.9409 & \cellcolor[HTML]{FDD37F}0.8083 & \cellcolor[HTML]{FDD07E}0.7970 & \cellcolor[HTML]{FEDA80}0.8346 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{6CC17C}0.9931 & \cellcolor[HTML]{6AC07C}0.9948 & \cellcolor[HTML]{65BF7C}0.9983 & \cellcolor[HTML]{80C77D}0.9800 & \cellcolor[HTML]{82C77D}0.9785 & \cellcolor[HTML]{79C57D}0.9847 & \cellcolor[HTML]{CDDD82}0.9277 & \cellcolor[HTML]{DBE182}0.9183 & \cellcolor[HTML]{B9D780}0.9414 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & Efficientnet\_b1 & \cellcolor[HTML]{67BF7C}0.9970 & \cellcolor[HTML]{6AC07C}0.9944 & \cellcolor[HTML]{6BC17C}0.9940 & \cellcolor[HTML]{78C57D}0.9849 & \cellcolor[HTML]{82C77D}0.9787 & \cellcolor[HTML]{7AC57D}0.9839 & \cellcolor[HTML]{C3DA81}0.9346 & \cellcolor[HTML]{D3DF82}0.9233 & \cellcolor[HTML]{BCD881}0.9390 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{67BF7C}0.9970 & \cellcolor[HTML]{68C07C}0.9957 & \cellcolor[HTML]{67C07C}0.9966 & \cellcolor[HTML]{80C77D}0.9796 & \cellcolor[HTML]{81C77D}0.9789 & \cellcolor[HTML]{7AC57D}0.9837 & \cellcolor[HTML]{C4DA81}0.9337 & \cellcolor[HTML]{CCDD82}0.9285 & \cellcolor[HTML]{B7D780}0.9425 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{\multirow{-5}{*}{Efficientnet\_b2}} & Swin\_s          & \cellcolor[HTML]{9CCF7F}0.9609 & \cellcolor[HTML]{8AC97E}0.9733 & \cellcolor[HTML]{86C87D}0.9759 & \cellcolor[HTML]{E9E583}0.9086 & \cellcolor[HTML]{C6DB81}0.9327 & \cellcolor[HTML]{BBD881}0.9398 & \cellcolor[HTML]{FDD37F}0.8074 & \cellcolor[HTML]{FED880}0.8265 & \cellcolor[HTML]{FEE082}0.8564 \\ \cline{2-12} 
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & ViT\_b\_16       & \cellcolor[HTML]{86C97E}0.9755 & \cellcolor[HTML]{89C97E}0.9735 & \cellcolor[HTML]{7DC67D}0.9819 & \cellcolor[HTML]{C9DC81}0.9306 & \cellcolor[HTML]{DAE182}0.9191 & \cellcolor[HTML]{B2D580}0.9460 & \cellcolor[HTML]{FDD27F}0.8029 & \cellcolor[HTML]{FDCE7E}0.7900 & \cellcolor[HTML]{FED980}0.8292 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{6CC17C}0.9932 & \cellcolor[HTML]{6DC17C}0.9928 & \cellcolor[HTML]{6AC17C}0.9944 & \cellcolor[HTML]{87C97E}0.9751 & \cellcolor[HTML]{84C87D}0.9773 & \cellcolor[HTML]{7DC67D}0.9815 & \cellcolor[HTML]{CEDD82}0.9271 & \cellcolor[HTML]{DEE283}0.9164 & \cellcolor[HTML]{C3DA81}0.9345 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & Efficientnet\_b2 & \cellcolor[HTML]{73C37C}0.9888 & \cellcolor[HTML]{70C27C}0.9904 & \cellcolor[HTML]{70C27C}0.9904 & \cellcolor[HTML]{95CD7E}0.9659 & \cellcolor[HTML]{9ACE7F}0.9619 & \cellcolor[HTML]{8FCB7E}0.9699 & \cellcolor[HTML]{FEE883}0.8832 & \cellcolor[HTML]{FEE583}0.8749 & \cellcolor[HTML]{FEEA83}0.8910 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & Resnet34         & \cellcolor[HTML]{65BF7C}0.9980 & \cellcolor[HTML]{69C07C}0.9952 & \cellcolor[HTML]{65BF7C}0.9980 & \cellcolor[HTML]{73C37C}0.9884 & \cellcolor[HTML]{78C47D}0.9854 & \cellcolor[HTML]{6DC17C}0.9924 & \cellcolor[HTML]{B5D680}0.9437 & \cellcolor[HTML]{C0D981}0.9365 & \cellcolor[HTML]{AED480}0.9485 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{\multirow{-5}{*}{Resnet18}}         & Swin\_s          & \cellcolor[HTML]{92CC7E}0.9675 & \cellcolor[HTML]{8ACA7E}0.9731 & \cellcolor[HTML]{7FC67D}0.9803 & \cellcolor[HTML]{E4E483}0.9119 & \cellcolor[HTML]{CBDC81}0.9288 & \cellcolor[HTML]{BBD881}0.9396 & \cellcolor[HTML]{FDCF7E}0.7942 & \cellcolor[HTML]{FDD680}0.8178 & \cellcolor[HTML]{FEDE81}0.8464 \\ \cline{2-12} 
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & ViT\_b\_16       & \cellcolor[HTML]{BDD881}0.9383 & \cellcolor[HTML]{B6D680}0.9429 & \cellcolor[HTML]{B2D580}0.9462 & \cellcolor[HTML]{FEE783}0.8820 & \cellcolor[HTML]{FEE683}0.8774 & \cellcolor[HTML]{F7E984}0.8995 & \cellcolor[HTML]{FDCA7D}0.7749 & \cellcolor[HTML]{FDC87D}0.7682 & \cellcolor[HTML]{FDD17F}0.7986 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{6AC07C}0.9945 & \cellcolor[HTML]{6DC17C}0.9926 & \cellcolor[HTML]{68C07C}0.9959 & \cellcolor[HTML]{7DC67D}0.9816 & \cellcolor[HTML]{82C77D}0.9781 & \cellcolor[HTML]{79C57D}0.9848 & \cellcolor[HTML]{C7DB81}0.9320 & \cellcolor[HTML]{DAE182}0.9191 & \cellcolor[HTML]{B7D780}0.9425 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & Efficientnet\_b2 & \cellcolor[HTML]{79C57D}0.9848 & \cellcolor[HTML]{73C37C}0.9885 & \cellcolor[HTML]{72C37C}0.9890 & \cellcolor[HTML]{A1D07F}0.9572 & \cellcolor[HTML]{A2D17F}0.9565 & \cellcolor[HTML]{9ACE7F}0.9620 & \cellcolor[HTML]{FEE883}0.8826 & \cellcolor[HTML]{FEE883}0.8841 & \cellcolor[HTML]{FEEB84}0.8946 \\
\multicolumn{1}{|l|}{}                            & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{68C07C}0.9963 & \cellcolor[HTML]{66BF7C}0.9977 & \cellcolor[HTML]{63BE7B}0.9991 & \cellcolor[HTML]{74C37C}0.9878 & \cellcolor[HTML]{7CC67D}0.9823 & \cellcolor[HTML]{72C37C}0.9890 & \cellcolor[HTML]{B0D580}0.9472 & \cellcolor[HTML]{BCD881}0.9393 & \cellcolor[HTML]{A3D17F}0.9559 \\
\multicolumn{1}{|l|}{\multirow{-25}{*}{Imagenet}} & \multicolumn{1}{c|}{\multirow{-5}{*}{Swin\_s}}          & Swin\_t          & \cellcolor[HTML]{6AC07C}0.9949 & \cellcolor[HTML]{6AC07C}0.9945 & \cellcolor[HTML]{6AC07C}0.9949 & \cellcolor[HTML]{7BC57D}0.9834 & \cellcolor[HTML]{89C97E}0.9740 & \cellcolor[HTML]{83C87D}0.9775 & \cellcolor[HTML]{B5D680}0.9438 & \cellcolor[HTML]{D6E082}0.9213 & \cellcolor[HTML]{D3DF82}0.9235 \\ \hline
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{99CE7F}0.9628 & \cellcolor[HTML]{9FD07F}0.9587 & \cellcolor[HTML]{A8D27F}0.9525 & \cellcolor[HTML]{B0D580}0.9474 & \cellcolor[HTML]{BBD881}0.9401 & \cellcolor[HTML]{CBDC81}0.9288 & \cellcolor[HTML]{CFDE82}0.9262 & \cellcolor[HTML]{D4DF82}0.9226 & \cellcolor[HTML]{FEEB84}0.8942 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{FEDD81}0.8430 & \cellcolor[HTML]{FDCB7D}0.7769 & \cellcolor[HTML]{FEE983}0.8884 & \cellcolor[HTML]{FCC07B}0.7368 & \cellcolor[HTML]{FBAA77}0.6553 & \cellcolor[HTML]{FDD17F}0.7998 & \cellcolor[HTML]{FA9774}0.5888 & \cellcolor[HTML]{F8756D}0.4644 & \cellcolor[HTML]{FBAC78}0.6662 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & EfficientNetB0   & \cellcolor[HTML]{F5E884}0.9008 & \cellcolor[HTML]{FEDD81}0.8450 & \cellcolor[HTML]{E5E483}0.9112 & \cellcolor[HTML]{FDD57F}0.8132 & \cellcolor[HTML]{FDC57C}0.7575 & \cellcolor[HTML]{FEDF81}0.8524 & \cellcolor[HTML]{FCB679}0.7007 & \cellcolor[HTML]{FA9A74}0.5975 & \cellcolor[HTML]{FDC77D}0.7616 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ResNet18         & \cellcolor[HTML]{FEDC81}0.8388 & \cellcolor[HTML]{FCB77A}0.7045 & \cellcolor[HTML]{FEE382}0.8678 & \cellcolor[HTML]{FCBF7B}0.7327 & \cellcolor[HTML]{FA9273}0.5707 & \cellcolor[HTML]{FDCE7E}0.7874 & \cellcolor[HTML]{FA9773}0.5882 & \cellcolor[HTML]{F8696B}0.4169 & \cellcolor[HTML]{FBAB77}0.6594 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{\multirow{-5}{*}{ViT}}              & swin\_s          & \cellcolor[HTML]{FEE081}0.8533 & \cellcolor[HTML]{FDD57F}0.8161 & \cellcolor[HTML]{FEE582}0.8719 & \cellcolor[HTML]{FDCD7E}0.7864 & \cellcolor[HTML]{FDC77D}0.7616 & \cellcolor[HTML]{FDD27F}0.8039 & \cellcolor[HTML]{FCB679}0.7023 & \cellcolor[HTML]{FBA376}0.6326 & \cellcolor[HTML]{FCB97A}0.7121 \\ \cline{2-12} 
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{FCBE7B}0.7289 & \cellcolor[HTML]{FDD17F}0.8012 & \cellcolor[HTML]{FDC67D}0.7610 & \cellcolor[HTML]{FCB87A}0.7078 & \cellcolor[HTML]{FCC37C}0.7470 & \cellcolor[HTML]{FCB579}0.6968 & \cellcolor[HTML]{FAA075}0.6202 & \cellcolor[HTML]{FA9F75}0.6182 & \cellcolor[HTML]{FAA075}0.6197 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{C7DB81}0.9317 & \cellcolor[HTML]{E5E483}0.9116 & \cellcolor[HTML]{FEE983}0.8876 & \cellcolor[HTML]{FEE282}0.8635 & \cellcolor[HTML]{FED980}0.8303 & \cellcolor[HTML]{FDD47F}0.8102 & \cellcolor[HTML]{FDC67D}0.7602 & \cellcolor[HTML]{FBB078}0.6804 & \cellcolor[HTML]{FCBB7A}0.7180 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & EfficientNetB0   & \cellcolor[HTML]{FEE883}0.8855 & \cellcolor[HTML]{FEE582}0.8715 & \cellcolor[HTML]{FEE983}0.8896 & \cellcolor[HTML]{FDD37F}0.8062 & \cellcolor[HTML]{FDCB7D}0.7781 & \cellcolor[HTML]{FDD37F}0.8072 & \cellcolor[HTML]{FCB479}0.6929 & \cellcolor[HTML]{FBA476}0.6337 & \cellcolor[HTML]{FCBA7A}0.7140 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ResNet18         & \cellcolor[HTML]{FDD57F}0.8133 & \cellcolor[HTML]{FDCD7E}0.7851 & \cellcolor[HTML]{FDD47F}0.8112 & \cellcolor[HTML]{FCBC7B}0.7239 & \cellcolor[HTML]{FBB078}0.6797 & \cellcolor[HTML]{FCC07B}0.7359 & \cellcolor[HTML]{FBA576}0.6397 & \cellcolor[HTML]{FA9072}0.5600 & \cellcolor[HTML]{FBA676}0.6407 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{\multirow{-5}{*}{DenseNet121}}      & swin\_s          & \cellcolor[HTML]{FEDC81}0.8414 & \cellcolor[HTML]{FDD27F}0.8032 & \cellcolor[HTML]{FEE182}0.8574 & \cellcolor[HTML]{FCC47C}0.7510 & \cellcolor[HTML]{FCB579}0.6978 & \cellcolor[HTML]{FDC87D}0.7681 & \cellcolor[HTML]{FBA276}0.6292 & \cellcolor[HTML]{FA8E72}0.5554 & \cellcolor[HTML]{FBAB77}0.6603 \\ \cline{2-12} 
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{FCC57C}0.7555 & \cellcolor[HTML]{FDD37F}0.8076 & \cellcolor[HTML]{FDC87D}0.7655 & \cellcolor[HTML]{FCB87A}0.7074 & \cellcolor[HTML]{FCBF7B}0.7345 & \cellcolor[HTML]{FCBC7B}0.7244 & \cellcolor[HTML]{FA9E75}0.6137 & \cellcolor[HTML]{FA9C74}0.6062 & \cellcolor[HTML]{FBA376}0.6328 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{FEE783}0.8818 & \cellcolor[HTML]{F6E984}0.8998 & \cellcolor[HTML]{FEE582}0.8737 & \cellcolor[HTML]{FDD37F}0.8076 & \cellcolor[HTML]{FED880}0.8267 & \cellcolor[HTML]{FDD37F}0.8056 & \cellcolor[HTML]{FCB679}0.6994 & \cellcolor[HTML]{FBB078}0.6784 & \cellcolor[HTML]{FBB179}0.6839 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & EfficientNetB0   & \cellcolor[HTML]{A3D17F}0.9559 & \cellcolor[HTML]{8CCA7E}0.9719 & \cellcolor[HTML]{C1D981}0.9359 & \cellcolor[HTML]{E1E383}0.9138 & \cellcolor[HTML]{C2DA81}0.9349 & \cellcolor[HTML]{F8E984}0.8988 & \cellcolor[HTML]{FEE082}0.8567 & \cellcolor[HTML]{FEE482}0.8697 & \cellcolor[HTML]{FDD67F}0.8166 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ResNet18         & \cellcolor[HTML]{FFEB84}0.8938 & \cellcolor[HTML]{D9E082}0.9198 & \cellcolor[HTML]{FFEB84}0.8938 & \cellcolor[HTML]{FDD47F}0.8126 & \cellcolor[HTML]{FEDC81}0.8387 & \cellcolor[HTML]{FED880}0.8267 & \cellcolor[HTML]{FCBA7A}0.7159 & \cellcolor[HTML]{FCB87A}0.7069 & \cellcolor[HTML]{FCBA7A}0.7174 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{\multirow{-5}{*}{EfficientNetB0}}   & swin\_s          & \cellcolor[HTML]{FEDB80}0.8357 & \cellcolor[HTML]{FEDD81}0.8457 & \cellcolor[HTML]{FEE081}0.8537 & \cellcolor[HTML]{FDC87D}0.7655 & \cellcolor[HTML]{FCC37C}0.7495 & \cellcolor[HTML]{FDCC7E}0.7806 & \cellcolor[HTML]{FBAA77}0.6553 & \cellcolor[HTML]{FA9C74}0.6052 & \cellcolor[HTML]{FBAD78}0.6698 \\ \cline{2-12} 
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{FCC37C}0.7475 & \cellcolor[HTML]{FDCC7E}0.7816 & \cellcolor[HTML]{FDCF7E}0.7936 & \cellcolor[HTML]{FCBA7A}0.7164 & \cellcolor[HTML]{FCC27C}0.7435 & \cellcolor[HTML]{FCBC7A}0.7214 & \cellcolor[HTML]{FA9B74}0.6014 & \cellcolor[HTML]{FA9D75}0.6109 & \cellcolor[HTML]{FA9F75}0.6179 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{FDCB7E}0.7796 & \cellcolor[HTML]{FCC37C}0.7475 & \cellcolor[HTML]{FDCF7E}0.7916 & \cellcolor[HTML]{FBAE78}0.6703 & \cellcolor[HTML]{FBA776}0.6453 & \cellcolor[HTML]{FCB77A}0.7054 & \cellcolor[HTML]{FA9172}0.5653 & \cellcolor[HTML]{F98570}0.5198 & \cellcolor[HTML]{FA9874}0.5899 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & EfficientNetB0   & \cellcolor[HTML]{FEDB80}0.8357 & \cellcolor[HTML]{FEDB80}0.8357 & \cellcolor[HTML]{FEE983}0.8878 & \cellcolor[HTML]{FDC97D}0.7715 & \cellcolor[HTML]{FCC57C}0.7555 & \cellcolor[HTML]{FDD47F}0.8096 & \cellcolor[HTML]{FBAD78}0.6690 & \cellcolor[HTML]{FBA175}0.6239 & \cellcolor[HTML]{FCB579}0.6975 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ResNet18         & \cellcolor[HTML]{FEE282}0.8637 & \cellcolor[HTML]{FEE182}0.8577 & \cellcolor[HTML]{FEE983}0.8898 & \cellcolor[HTML]{FDCD7E}0.7846 & \cellcolor[HTML]{FCC47C}0.7535 & \cellcolor[HTML]{FDD37F}0.8056 & \cellcolor[HTML]{FBA676}0.6420 & \cellcolor[HTML]{FA9B74}0.6034 & \cellcolor[HTML]{FBB279}0.6880 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{\multirow{-5}{*}{ResNet18}}         & swin\_s          & \cellcolor[HTML]{FDD37F}0.8076 & \cellcolor[HTML]{FDD17F}0.7996 & \cellcolor[HTML]{FEDC81}0.8397 & \cellcolor[HTML]{FCC07B}0.7385 & \cellcolor[HTML]{FCB479}0.6954 & \cellcolor[HTML]{FDC97D}0.7705 & \cellcolor[HTML]{FA9B74}0.6029 & \cellcolor[HTML]{F98B71}0.5443 & \cellcolor[HTML]{FBA676}0.6410 \\ \cline{2-12} 
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{FCC17C}0.7428 & \cellcolor[HTML]{FDD780}0.8210 & \cellcolor[HTML]{FCC47C}0.7531 & \cellcolor[HTML]{FCB679}0.7020 & \cellcolor[HTML]{FCC27C}0.7451 & \cellcolor[HTML]{FCB77A}0.7030 & \cellcolor[HTML]{FBA276}0.6292 & \cellcolor[HTML]{FBAC77}0.6626 & \cellcolor[HTML]{FBA476}0.6359 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{FDEB84}0.8951 & \cellcolor[HTML]{FEE583}0.8745 & \cellcolor[HTML]{F1E784}0.9033 & \cellcolor[HTML]{FDCF7E}0.7934 & \cellcolor[HTML]{FDC87D}0.7677 & \cellcolor[HTML]{FED980}0.8294 & \cellcolor[HTML]{FCB479}0.6929 & \cellcolor[HTML]{FA9B74}0.6004 & \cellcolor[HTML]{FCBD7B}0.7257 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & EfficientNetB0   & \cellcolor[HTML]{EBE683}0.9074 & \cellcolor[HTML]{F1E784}0.9033 & \cellcolor[HTML]{DFE283}0.9156 & \cellcolor[HTML]{FEE282}0.8613 & \cellcolor[HTML]{FEDC81}0.8417 & \cellcolor[HTML]{FEE482}0.8684 & \cellcolor[HTML]{FDCD7E}0.7838 & \cellcolor[HTML]{FCB97A}0.7119 & \cellcolor[HTML]{FDD07E}0.7971 \\
\multicolumn{1}{|c|}{}                            & \multicolumn{1}{c|}{}                                   & ResNet18         & \cellcolor[HTML]{FEE182}0.8580 & \cellcolor[HTML]{FDD780}0.8210 & \cellcolor[HTML]{FEE583}0.8745 & \cellcolor[HTML]{FDC77D}0.7646 & \cellcolor[HTML]{FCB579}0.6989 & \cellcolor[HTML]{FDD680}0.8201 & \cellcolor[HTML]{FBAC77}0.6631 & \cellcolor[HTML]{F98A71}0.5388 & \cellcolor[HTML]{FCB579}0.6965 \\
\multicolumn{1}{|c|}{\multirow{-25}{*}{Cifar}}    & \multicolumn{1}{c|}{\multirow{-5}{*}{swin\_s}}          & swin\_s          & \cellcolor[HTML]{90CB7E}0.9691 & \cellcolor[HTML]{9FD07F}0.9588 & \cellcolor[HTML]{ABD380}0.9506 & \cellcolor[HTML]{B3D580}0.9455 & \cellcolor[HTML]{E2E383}0.9137 & \cellcolor[HTML]{E9E583}0.9085 & \cellcolor[HTML]{FEEA83}0.8932 & \cellcolor[HTML]{FEDD81}0.8428 & \cellcolor[HTML]{FEDD81}0.8423 \\ \hline
\end{tabular}
}
\end{table}

==> tables/transforms_road_sign_xray.tex <==
\begin{table}[]
\resizebox{\linewidth}{!}{%
\begin{tabular}{|lccc|lll|lll|lll|}
\hline
\multicolumn{2}{|l}{}                                                                              &                                                         &                  & \multicolumn{3}{c|}{@5\%}                                                                     & \multicolumn{3}{c|}{@10\%}                                                                    & \multicolumn{3}{c|}{@20\%}                                                                    \\ \cline{5-13} 
\multicolumn{2}{|l}{}                                                                              & Surrogate                                               & Victim           & \multicolumn{1}{c}{Resize}    & \multicolumn{1}{c}{Comp}      & \multicolumn{1}{c|}{Comb}     & \multicolumn{1}{c}{Resize}    & \multicolumn{1}{c}{Comp}      & \multicolumn{1}{c|}{Comb}     & \multicolumn{1}{c}{Resize}    & \multicolumn{1}{c}{Comp}      & \multicolumn{1}{c|}{Comb}     \\ \hline
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{71C27C}0.976 & \cellcolor[HTML]{71C27C}0.976 & \cellcolor[HTML]{71C27C}0.976 & \cellcolor[HTML]{84C87D}0.943 & \cellcolor[HTML]{84C87D}0.943 & \cellcolor[HTML]{84C87D}0.943 & \cellcolor[HTML]{9CCF7F}0.900 & \cellcolor[HTML]{9CCF7F}0.900 & \cellcolor[HTML]{9CCF7F}0.900 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{8ACA7E}0.931 & \cellcolor[HTML]{8ACA7E}0.931 & \cellcolor[HTML]{8ACA7E}0.931 & \cellcolor[HTML]{B0D580}0.863 & \cellcolor[HTML]{B0D580}0.863 & \cellcolor[HTML]{B0D580}0.863 & \cellcolor[HTML]{F2E884}0.746 & \cellcolor[HTML]{F2E884}0.746 & \cellcolor[HTML]{F2E884}0.746 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet\_b2 & \cellcolor[HTML]{7DC67D}0.955 & \cellcolor[HTML]{7DC67D}0.955 & \cellcolor[HTML]{7DC67D}0.955 & \cellcolor[HTML]{9DCF7F}0.898 & \cellcolor[HTML]{9DCF7F}0.898 & \cellcolor[HTML]{9DCF7F}0.898 & \cellcolor[HTML]{E3E383}0.774 & \cellcolor[HTML]{E3E383}0.774 & \cellcolor[HTML]{E3E383}0.774 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{84C87D}0.943 & \cellcolor[HTML]{84C87D}0.943 & \cellcolor[HTML]{84C87D}0.943 & \cellcolor[HTML]{A5D27F}0.883 & \cellcolor[HTML]{A5D27F}0.883 & \cellcolor[HTML]{A5D27F}0.883 & \cellcolor[HTML]{EAE583}0.761 & \cellcolor[HTML]{EAE583}0.761 & \cellcolor[HTML]{EAE583}0.761 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{\multirow{-5}{*}{ViT}}              & Swin\_s          & \cellcolor[HTML]{82C77D}0.946 & \cellcolor[HTML]{82C77D}0.946 & \cellcolor[HTML]{82C77D}0.946 & \cellcolor[HTML]{9BCF7F}0.901 & \cellcolor[HTML]{9BCF7F}0.901 & \cellcolor[HTML]{9BCF7F}0.901 & \cellcolor[HTML]{D9E082}0.791 & \cellcolor[HTML]{D9E082}0.791 & \cellcolor[HTML]{D9E082}0.791 \\ \cline{3-13} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{A4D17F}0.885 & \cellcolor[HTML]{A4D17F}0.885 & \cellcolor[HTML]{A4D17F}0.885 & \cellcolor[HTML]{C1D981}0.834 & \cellcolor[HTML]{C1D981}0.834 & \cellcolor[HTML]{C1D981}0.834 & \cellcolor[HTML]{FEE883}0.707 & \cellcolor[HTML]{FEE883}0.707 & \cellcolor[HTML]{FEE883}0.707 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{6AC07C}0.989 & \cellcolor[HTML]{6AC07C}0.989 & \cellcolor[HTML]{6AC07C}0.989 & \cellcolor[HTML]{69C07C}0.991 & \cellcolor[HTML]{69C07C}0.991 & \cellcolor[HTML]{69C07C}0.991 & \cellcolor[HTML]{69C07C}0.990 & \cellcolor[HTML]{69C07C}0.990 & \cellcolor[HTML]{69C07C}0.990 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet\_b2 & \cellcolor[HTML]{89C97E}0.933 & \cellcolor[HTML]{89C97E}0.933 & \cellcolor[HTML]{89C97E}0.933 & \cellcolor[HTML]{9DCF7F}0.898 & \cellcolor[HTML]{9DCF7F}0.898 & \cellcolor[HTML]{9DCF7F}0.898 & \cellcolor[HTML]{B6D680}0.852 & \cellcolor[HTML]{B6D680}0.852 & \cellcolor[HTML]{B6D680}0.852 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{6EC17C}0.981 & \cellcolor[HTML]{6EC17C}0.981 & \cellcolor[HTML]{6EC17C}0.981 & \cellcolor[HTML]{8ACA7E}0.932 & \cellcolor[HTML]{8ACA7E}0.932 & \cellcolor[HTML]{8ACA7E}0.932 & \cellcolor[HTML]{A8D27F}0.878 & \cellcolor[HTML]{A8D27F}0.878 & \cellcolor[HTML]{A8D27F}0.878 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{\multirow{-5}{*}{DenseNet121}}      & Swin\_s          & \cellcolor[HTML]{87C97E}0.937 & \cellcolor[HTML]{87C97E}0.937 & \cellcolor[HTML]{87C97E}0.937 & \cellcolor[HTML]{9ACE7F}0.902 & \cellcolor[HTML]{9ACE7F}0.902 & \cellcolor[HTML]{9ACE7F}0.902 & \cellcolor[HTML]{D2DF82}0.802 & \cellcolor[HTML]{D2DF82}0.802 & \cellcolor[HTML]{D2DF82}0.802 \\ \cline{3-13} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{9FD07F}0.893 & \cellcolor[HTML]{9FD07F}0.893 & \cellcolor[HTML]{9FD07F}0.893 & \cellcolor[HTML]{D4DF82}0.800 & \cellcolor[HTML]{D4DF82}0.800 & \cellcolor[HTML]{D4DF82}0.800 & \cellcolor[HTML]{FEE582}0.691 & \cellcolor[HTML]{FEE582}0.691 & \cellcolor[HTML]{FEE582}0.691 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{83C87D}0.943 & \cellcolor[HTML]{83C87D}0.943 & \cellcolor[HTML]{83C87D}0.943 & \cellcolor[HTML]{9DCF7F}0.897 & \cellcolor[HTML]{9DCF7F}0.897 & \cellcolor[HTML]{9DCF7F}0.897 & \cellcolor[HTML]{D0DE82}0.807 & \cellcolor[HTML]{D0DE82}0.807 & \cellcolor[HTML]{D0DE82}0.807 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet\_b2 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{85C87D}0.940 & \cellcolor[HTML]{85C87D}0.940 & \cellcolor[HTML]{85C87D}0.940 & \cellcolor[HTML]{9DCF7F}0.897 & \cellcolor[HTML]{9DCF7F}0.897 & \cellcolor[HTML]{9DCF7F}0.897 & \cellcolor[HTML]{C8DC81}0.820 & \cellcolor[HTML]{C8DC81}0.820 & \cellcolor[HTML]{C8DC81}0.820 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{\multirow{-5}{*}{Efficientnet\_b2}} & Swin\_s          & \cellcolor[HTML]{89C97E}0.933 & \cellcolor[HTML]{89C97E}0.933 & \cellcolor[HTML]{89C97E}0.933 & \cellcolor[HTML]{A5D17F}0.883 & \cellcolor[HTML]{A5D17F}0.883 & \cellcolor[HTML]{A5D17F}0.883 & \cellcolor[HTML]{E2E383}0.774 & \cellcolor[HTML]{E2E383}0.774 & \cellcolor[HTML]{E2E383}0.774 \\ \cline{3-13} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{A0D07F}0.892 & \cellcolor[HTML]{A0D07F}0.892 & \cellcolor[HTML]{A0D07F}0.892 & \cellcolor[HTML]{CFDD82}0.809 & \cellcolor[HTML]{CFDD82}0.809 & \cellcolor[HTML]{CFDD82}0.809 & \cellcolor[HTML]{FEE282}0.677 & \cellcolor[HTML]{FEE282}0.677 & \cellcolor[HTML]{FEE282}0.677 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{7CC67D}0.956 & \cellcolor[HTML]{7CC67D}0.956 & \cellcolor[HTML]{7CC67D}0.956 & \cellcolor[HTML]{8CCA7E}0.927 & \cellcolor[HTML]{8CCA7E}0.927 & \cellcolor[HTML]{8CCA7E}0.927 & \cellcolor[HTML]{AED480}0.867 & \cellcolor[HTML]{AED480}0.867 & \cellcolor[HTML]{AED480}0.867 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet\_b2 & \cellcolor[HTML]{7AC57D}0.959 & \cellcolor[HTML]{7AC57D}0.959 & \cellcolor[HTML]{7AC57D}0.959 & \cellcolor[HTML]{8ECB7E}0.924 & \cellcolor[HTML]{8ECB7E}0.924 & \cellcolor[HTML]{8ECB7E}0.924 & \cellcolor[HTML]{AAD380}0.875 & \cellcolor[HTML]{AAD380}0.875 & \cellcolor[HTML]{AAD380}0.875 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{\multirow{-5}{*}{Resnet18}}         & Swin\_s          & \cellcolor[HTML]{93CC7E}0.916 & \cellcolor[HTML]{93CC7E}0.916 & \cellcolor[HTML]{93CC7E}0.916 & \cellcolor[HTML]{A1D07F}0.890 & \cellcolor[HTML]{A1D07F}0.890 & \cellcolor[HTML]{A1D07F}0.890 & \cellcolor[HTML]{D7E082}0.794 & \cellcolor[HTML]{D7E082}0.794 & \cellcolor[HTML]{D7E082}0.794 \\ \cline{3-13} 
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{9DCF7F}0.898 & \cellcolor[HTML]{9DCF7F}0.898 & \cellcolor[HTML]{9DCF7F}0.898 & \cellcolor[HTML]{DAE182}0.789 & \cellcolor[HTML]{DAE182}0.789 & \cellcolor[HTML]{DAE182}0.789 & \cellcolor[HTML]{FEDD81}0.645 & \cellcolor[HTML]{FEDD81}0.645 & \cellcolor[HTML]{FEDD81}0.645 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{79C57D}0.961 & \cellcolor[HTML]{79C57D}0.961 & \cellcolor[HTML]{79C57D}0.961 & \cellcolor[HTML]{98CE7F}0.907 & \cellcolor[HTML]{98CE7F}0.907 & \cellcolor[HTML]{98CE7F}0.907 & \cellcolor[HTML]{D7E082}0.795 & \cellcolor[HTML]{D7E082}0.795 & \cellcolor[HTML]{D7E082}0.795 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet\_b2 & \cellcolor[HTML]{71C27C}0.976 & \cellcolor[HTML]{71C27C}0.976 & \cellcolor[HTML]{71C27C}0.976 & \cellcolor[HTML]{93CC7E}0.916 & \cellcolor[HTML]{93CC7E}0.916 & \cellcolor[HTML]{93CC7E}0.916 & \cellcolor[HTML]{BFD981}0.836 & \cellcolor[HTML]{BFD981}0.836 & \cellcolor[HTML]{BFD981}0.836 \\
\multicolumn{1}{|c|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{78C47D}0.964 & \cellcolor[HTML]{78C47D}0.964 & \cellcolor[HTML]{78C47D}0.964 & \cellcolor[HTML]{97CD7E}0.909 & \cellcolor[HTML]{97CD7E}0.909 & \cellcolor[HTML]{97CD7E}0.909 & \cellcolor[HTML]{D3DF82}0.801 & \cellcolor[HTML]{D3DF82}0.801 & \cellcolor[HTML]{D3DF82}0.801 \\
\multicolumn{1}{|c|}{\multirow{-25}{*}{X-ray}} & \multicolumn{1}{c|}{\multirow{-25}{*}{X-Ray}}     & \multicolumn{1}{c|}{\multirow{-5}{*}{Swin\_s}}          & Swin\_s          & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{63BE7B}1.000 & \cellcolor[HTML]{64BF7C}0.999 & \cellcolor[HTML]{64BF7C}0.999 & \cellcolor[HTML]{64BF7C}0.999 \\ \hline
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8796E}0.091 & \cellcolor[HTML]{F8796E}0.091 & \cellcolor[HTML]{F8796E}0.091 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8796E}0.091 & \cellcolor[HTML]{F8796E}0.091 & \cellcolor[HTML]{F8796E}0.091 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet\_b2 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F98D71}0.200 & \cellcolor[HTML]{F98D71}0.200 & \cellcolor[HTML]{F98D71}0.200 & \cellcolor[HTML]{FBAA77}0.364 & \cellcolor[HTML]{FBAA77}0.364 & \cellcolor[HTML]{FBAA77}0.364 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8796E}0.091 & \cellcolor[HTML]{F8796E}0.091 & \cellcolor[HTML]{F8796E}0.091 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{\multirow{-5}{*}{ViT}}              & Swin\_s          & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{FA9A74}0.273 & \cellcolor[HTML]{FA9A74}0.273 & \cellcolor[HTML]{FA9A74}0.273 \\ \cline{3-13} 
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F86F6C}0.033 & \cellcolor[HTML]{F86F6C}0.033 & \cellcolor[HTML]{F86F6C}0.033 & \cellcolor[HTML]{F86C6B}0.017 & \cellcolor[HTML]{F86C6B}0.017 & \cellcolor[HTML]{F86C6B}0.017 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{FBA576}0.333 & \cellcolor[HTML]{FBA576}0.333 & \cellcolor[HTML]{FBA576}0.333 & \cellcolor[HTML]{FBAB77}0.367 & \cellcolor[HTML]{FBAB77}0.367 & \cellcolor[HTML]{FBAB77}0.367 & \cellcolor[HTML]{FBAB77}0.367 & \cellcolor[HTML]{FBAB77}0.367 & \cellcolor[HTML]{FBAB77}0.367 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet\_b2 & \cellcolor[HTML]{F8756D}0.067 & \cellcolor[HTML]{F8756D}0.067 & \cellcolor[HTML]{F8756D}0.067 & \cellcolor[HTML]{F9816F}0.133 & \cellcolor[HTML]{F9816F}0.133 & \cellcolor[HTML]{F9816F}0.133 & \cellcolor[HTML]{F98770}0.167 & \cellcolor[HTML]{F98770}0.167 & \cellcolor[HTML]{F98770}0.167 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F86F6C}0.033 & \cellcolor[HTML]{F86F6C}0.033 & \cellcolor[HTML]{F86F6C}0.033 & \cellcolor[HTML]{F86F6C}0.033 & \cellcolor[HTML]{F86F6C}0.033 & \cellcolor[HTML]{F86F6C}0.033 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{\multirow{-5}{*}{DenseNet121}}      & Swin\_s          & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F86F6C}0.033 & \cellcolor[HTML]{F86F6C}0.033 & \cellcolor[HTML]{F86F6C}0.033 & \cellcolor[HTML]{F8726C}0.050 & \cellcolor[HTML]{F8726C}0.050 & \cellcolor[HTML]{F8726C}0.050 \\ \cline{3-13} 
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F86E6C}0.032 & \cellcolor[HTML]{F86E6C}0.032 & \cellcolor[HTML]{F86E6C}0.032 & \cellcolor[HTML]{F86B6B}0.016 & \cellcolor[HTML]{F86B6B}0.016 & \cellcolor[HTML]{F86B6B}0.016 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F86E6C}0.032 & \cellcolor[HTML]{F86E6C}0.032 & \cellcolor[HTML]{F86E6C}0.032 & \cellcolor[HTML]{F86B6B}0.016 & \cellcolor[HTML]{F86B6B}0.016 & \cellcolor[HTML]{F86B6B}0.016 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet\_b2 & \cellcolor[HTML]{AED480}0.867 & \cellcolor[HTML]{AED480}0.867 & \cellcolor[HTML]{AED480}0.867 & \cellcolor[HTML]{ACD380}0.871 & \cellcolor[HTML]{ACD380}0.871 & \cellcolor[HTML]{ACD380}0.871 & \cellcolor[HTML]{B5D680}0.855 & \cellcolor[HTML]{B5D680}0.855 & \cellcolor[HTML]{B5D680}0.855 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F86E6C}0.032 & \cellcolor[HTML]{F86E6C}0.032 & \cellcolor[HTML]{F86E6C}0.032 & \cellcolor[HTML]{F86B6B}0.016 & \cellcolor[HTML]{F86B6B}0.016 & \cellcolor[HTML]{F86B6B}0.016 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{\multirow{-5}{*}{Efficientnet\_b2}} & Swin\_s          & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F86E6C}0.032 & \cellcolor[HTML]{F86E6C}0.032 & \cellcolor[HTML]{F86E6C}0.032 & \cellcolor[HTML]{F8716C}0.048 & \cellcolor[HTML]{F8716C}0.048 & \cellcolor[HTML]{F8716C}0.048 \\ \cline{3-13} 
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F86D6B}0.026 & \cellcolor[HTML]{F86D6B}0.026 & \cellcolor[HTML]{F86D6B}0.026 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F86D6B}0.026 & \cellcolor[HTML]{F86D6B}0.026 & \cellcolor[HTML]{F86D6B}0.026 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet\_b2 & \cellcolor[HTML]{F8726C}0.053 & \cellcolor[HTML]{F8726C}0.053 & \cellcolor[HTML]{F8726C}0.053 & \cellcolor[HTML]{F8776D}0.079 & \cellcolor[HTML]{F8776D}0.079 & \cellcolor[HTML]{F8776D}0.079 & \cellcolor[HTML]{F97B6E}0.104 & \cellcolor[HTML]{F97B6E}0.104 & \cellcolor[HTML]{F97B6E}0.104 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{F7E984}0.737 & \cellcolor[HTML]{F7E984}0.737 & \cellcolor[HTML]{F7E984}0.737 & \cellcolor[HTML]{FDD17F}0.579 & \cellcolor[HTML]{FDD17F}0.579 & \cellcolor[HTML]{FDD17F}0.579 & \cellcolor[HTML]{FCB87A}0.442 & \cellcolor[HTML]{FCB87A}0.442 & \cellcolor[HTML]{FCB87A}0.442 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{\multirow{-5}{*}{Resnet18}}         & Swin\_s          & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8706C}0.039 & \cellcolor[HTML]{F8706C}0.039 & \cellcolor[HTML]{F8706C}0.039 \\ \cline{3-13} 
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & ViT              & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F86D6B}0.024 & \cellcolor[HTML]{F86D6B}0.024 & \cellcolor[HTML]{F86D6B}0.024 & \cellcolor[HTML]{F86B6B}0.012 & \cellcolor[HTML]{F86B6B}0.012 & \cellcolor[HTML]{F86B6B}0.012 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & DenseNet121      & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F86D6B}0.024 & \cellcolor[HTML]{F86D6B}0.024 & \cellcolor[HTML]{F86D6B}0.024 & \cellcolor[HTML]{F86B6B}0.012 & \cellcolor[HTML]{F86B6B}0.012 & \cellcolor[HTML]{F86B6B}0.012 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Efficientnet\_b2 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8766D}0.073 & \cellcolor[HTML]{F8766D}0.073 & \cellcolor[HTML]{F8766D}0.073 & \cellcolor[HTML]{F8736D}0.060 & \cellcolor[HTML]{F8736D}0.060 & \cellcolor[HTML]{F8736D}0.060 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                   & Resnet18         & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8696B}0.000 & \cellcolor[HTML]{F8716C}0.049 & \cellcolor[HTML]{F8716C}0.049 & \cellcolor[HTML]{F8716C}0.049 & \cellcolor[HTML]{F86D6B}0.024 & \cellcolor[HTML]{F86D6B}0.024 & \cellcolor[HTML]{F86D6B}0.024 \\
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{c|}{\multirow{-25}{*}{Road Sign}} & \multicolumn{1}{c|}{\multirow{-5}{*}{Swin\_s}}          & Swin\_s          & \cellcolor[HTML]{FA9673}0.250 & \cellcolor[HTML]{FA9673}0.250 & \cellcolor[HTML]{FA9673}0.250 & \cellcolor[HTML]{FA9473}0.244 & \cellcolor[HTML]{FA9473}0.244 & \cellcolor[HTML]{FA9473}0.244 & \cellcolor[HTML]{FA9673}0.253 & \cellcolor[HTML]{FA9673}0.253 & \cellcolor[HTML]{FA9673}0.253 \\ \hline
\end{tabular}
}
\end{table}
